Temporal Enhanced Training of Multi-view 3D Object Detector via Historical Object Prediction

In this paper, we propose a new paradigm, named Historical Object Prediction (HoP) for multi-view 3D detection to leverage temporal information more effectively. The HoP approach is straightforward: given the current timestamp t, we generate a pseudo Bird's-Eye View (BEV) feature of timestamp t-k from its adjacent frames and utilize this feature to predict the object set at timestamp t-k. Our approach is motivated by the observation that enforcing the detector to capture both the spatial location and temporal motion of objects occurring at historical timestamps can lead to more accurate BEV feature learning. First, we elaborately design short-term and long-term temporal decoders, which can generate the pseudo BEV feature for timestamp t-k without the involvement of its corresponding camera images. Second, an additional object decoder is flexibly attached to predict the object targets using the generated pseudo BEV feature. Note that we only perform HoP during training, thus the proposed method does not introduce extra overheads during inference. As a plug-and-play approach, HoP can be easily incorporated into state-of-the-art BEV detection frameworks, including BEVFormer and BEVDet series. Furthermore, the auxiliary HoP approach is complementary to prevalent temporal modeling methods, leading to significant performance gains. Extensive experiments are conducted to evaluate the effectiveness of the proposed HoP on the nuScenes dataset. We choose the representative methods, including BEVFormer and BEVDet4D-Depth to evaluate our method. Surprisingly, HoP achieves 68.5% NDS and 62.4% mAP with ViT-L on nuScenes test, outperforming all the 3D object detectors on the leaderboard. Codes will be available at https://github.com/Sense-X/HoP.

==> tmp_method.tex <==
\section{Method}
\subsection{Overall Architecture}
Our method is built upon the optimized multi-view 3D object detector BEVFormer.
The image features of $6$ cameras are extracted and then lifted into the BEV feature by the BEV spatial encoder.
Multiple BEV features of different frames are fused by the BEV temporal encoder following~\cite{} but we do not warp these features.
Instead, we transform the extrinsic parameters of previous frames to the coordinate system of the current ego to perform the temporal alignment.
To further facilitate the temporal modeling of the BEV detector, we introduce an auxiliary training task to detect the 3D objects of the masked previous frame.
Note that the proposed training scheme only introduces extra overheads during training.
xxx

\subsection{Temporal Masked Objects Detection}
The architecture of our temporal masked objects detection is composed of an encoder $\mathcal{\hat{E}}$ and a decoder $\mathcal{\hat{D}}$.
Given the BEV feature sequence $\{\mathbf{B}_{t-N}, \cdots, \mathbf{B}_t\}$ that consists of $N$ previous frame features and the current BEV feature, we denote the  corresponding 3D ground truths as $\{\mathbf{G}_{t-N}, \cdots, \mathbf{G}_t\}$.
If the $k$-th previous BEV feature is discarded, we use the remainder BEV feature sequence $\{\mathbf{B}_{t-N}, \cdots, \mathbf{B}_t\} - \{\mathbf{B}_{t-k}\}$ (denoted as $\mathbf{B}^{rem}$) to predict the 3D ground truth $\mathbf{G}_{t-k}$ of previous frame $t-k$.
To be specific, we adopt $\mathcal{\hat{E}}$ and $\mathcal{\hat{D}}$ to transform the remainder BEV features to obtain the 3D predictions $\mathbf{\hat{P}}_{t-k}$ and minimize the differences between $\mathbf{\hat{P}}_{t-k}$ and $\mathbf{G}_{t-k}$.
\begin{equation}
    \label{eq:pred}
    \mathbf{\hat{P}}_{t-k} = \mathcal{D}(\mathcal{E}(\{\mathbf{B}_{t-N}, \cdots, \mathbf{B}_t\} - \{\mathbf{B}_{t-k}\})).
\end{equation}

% \noindent\textbf{Masked temporal encoder.}
% Given the mask index $k$ and masked BEV feature $\mathbf{B}_{t-k}$, 
The input to the temporal encoder is the remainder set of BEV features consisting of (i) previous BEV features $\{\mathbf{B}_{t-N}, \cdots, \mathbf{B}_{t-k-1}\}$, and
(ii) future BEV features $\{\mathbf{B}_{t-k+1}, \cdots, \mathbf{B}_{t}\}$. 
Our masked temporal encoder reconstructs the masked feature $\mathbf{\hat{B}}_{t-k}$ by utilizing the spatial semantics and temporal cues of the BEV feature sequence.
We first add temporal positional embeddings to BEV features in this full set to introduce the temporal location information.
To reconstruct the discarded BEV feature by both previous and future frames, we present a dual temporal decoder to capture both short-term and long-term information.

\noindent\textbf{Short-term temporal decoder.}
% the temporal difference between the reference and
% source frame varies significantly over different pixels, depths, cameras, and ego-motion.
% The temporal difference between the adjacent frames varies marginally thanks to the time interval.
Thanks to the marginal temporal difference between adjacent frames, the short-term temporal decoder only operates on the adjacent BEV feature set $\{\mathbf{B}_{t-k-1}, \mathbf{B}_{t-k+1}\}$ (denoted as $\mathbf{B}^{adj}$), building a detailed spatial representation.
We first define a grid-shaped learnable short-term BEV queries $\mathbf{Q}^{short}_{t-k} \in \mathbb{R}^{H \times W \times C}$, where $H$ and $W$ refer to the spatial shape of the BEV plane.
The short-term BEV queries aggregate the spatial information and model the short-term motion from $\mathbf{B}_{t-k-1}$ and $\mathbf{B}_{t-k+1}$ through the short-term temporal attention, which can be formulated as:
\begin{equation}
    \label{eq:short_term}
    \mathbf{\hat{B}}^{short}_{t-k} = \sum_{\mathbf{V} \in \mathbf{B}^{adj}} \mathrm{DeformAttn}(\mathbf{Q}^{short}_{t-k, p},p,\mathbf{V}),
\end{equation}
where $p$ is the spatial index in the BEV plane, $\mathrm{DeformAttn}(q,p,x)$ refers to the deformable attention with query $q$, reference point $p$ and input features $x$.
However, it is still challenging to precisely construct the temporal relations of the same objects between the discarded $\mathbf{B}_{t-k}$ and other BEV features with only two adjacent frames.

\noindent\textbf{Long-term temporal decoder.}
The long-term temporal decoder can be supplementary to the short-term temporal decoder, 
processing the whole remainder BEV set to perceive the motion clues over long-term history.
It is intuitive we only focus on the long-term \textit{spatial motion} of the same objects in the bird’s eye view, ignoring the height information that has been flattened into the channels.
Accordingly, we first employ a channel reduction operation to the remainder set $\mathbf{B}^{rem}$ to prune the height information while achieving better training efficiency.
Given the learnable long-term BEV queries $\mathbf{Q}^{long}_{t-k} \in \mathbb{R}^{H \times W \times C/r}$ and reduction layer with parameter $\mathbf{W}^{r} \in \mathbb{R}^{C \times C/r}$, we can capture the long-term dependencies as:
\begin{equation}
    \label{eq:long_term}
    \mathbf{\hat{B}}^{long}_{t-k} = \sum_{\mathbf{V} \in \mathbf{B}^{rem}} \mathrm{DeformAttn}(\mathbf{Q}^{short}_{t-k, p},p,\mathbf{V}\mathbf{W}^{r}),
\end{equation}
where $r$ denotes the reduction ratio.
Finally, we concatenate the short-term and long-term BEV features and perform feature fusion by a 3$\times$3 convolution layer.
% Note that we only focus on the spatial differences between frames in the bird’s eye view
% Note that we first employ a squeeze operation to
% capturing spatial motion without building a
% detailed spatial representation

\noindent\textbf{Object decoder.}
The reconstructed BEV feature $\mathbf{\hat{B}}_{t-k}$ is further processed by a lightweight object decoder.
% Note that the decoder is used to generate 3D predictions upon the BEV feature and thus can be flexibly implemented by any current BEV detection head.
% For example, we choose CenterPoint as the object decoder due to its simplicity.
% The implementation of this object decoder is flexible. 
The decoder is used to generate 3D predictions upon the BEV feature and thus its implementation is flexible.
Variants of BEV detection heads are an obvious choice and we will consider multiple instantiations in our experiments.

\noindent\textbf{Training objective.}
Considering the ego motion, 3D coordinates of the ground truth in frame $t-k$ should be transformed into the coordinate system of the current frame $t$.
Accordingly, we convert $\mathbf{G}_{t-k}$ to $\mathbf{\hat{G}}_{t-k}$ by ego transformation matrix and the training objective of the temporal masked objects detection task can be illustrated as:
\begin{equation}
    \label{eq:objective}
    \mathcal{L}_{pred} = \mathcal{L}_{3d}(\mathbf{\hat{P}}_{t-k}, \mathbf{\hat{G}}_{t-k}),
\end{equation}
where $\mathcal{L}_{3d}$ is the 3D object detection loss.



%%%%%%%%%%%%%%%%%%%%% original
\subsection{Temporal Query Fusion}
Object queries output by the BEV detector are used to predict 3D bounding boxes, and therefore they have filtered out noisy background information in BEV features. To explicitly leverage this instance-level prior information, we propose to reuse object queries derived from history BEV features. 

\noindent\textbf{Query fusion form.} The BEV feature sequences $\{\mathbf{B}_{t-N}, \cdots, \mathbf{B}_t\}$ are inferred in the time order. The object queries $\mathbf{O}$ are input into decoder $\mathcal{D}$ and outputs $\mathbf{\bar{O}}$. For the timestamp $t-k$, the process can be illustrated as:
\begin{equation}
    \label{eq:qpred}
    \mathbf{\bar{O}}_{t-k} = \mathcal{D}(\mathbf{B}_{t-k},\mathbf{O}_{t-k})
\end{equation}

The query fusion aims to supply specific temporal information for each query, which follows an intuition that current queries could therefore obtain better initialization with an awareness of historical perception. Specifically, to infer on the BEV feature $\mathbf{B}_{t-k}$, we collect aggregated previous object queries $\mathbf{O}^{his}_{t-k}$ according to the form of query connection, and then merge them with current object queries $\mathbf{O}_{t-k}$ as Eqn. \ref{eq:sum},
\begin{equation}
    \label{eq:sum}
    \mathbf{\bar{O}}_{t-k} = \mathcal{D}(\mathbf{B}_{t-k},\mathrm{Merge}(\mathbf{O}_{t-k},\mathbf{O}^{his}_{t-k}))
\end{equation}
where $\mathrm{Merge}$ is a merge function, e.g., a cross-attention layer.

\noindent\textbf{Query connection forms.}
The query connection forms determine how to derive aggregated history object queries $\mathbf{O}^{his}_{t-k}$ from history object queries $\{\mathbf{\bar{O}}_{t-N}, ..., \mathbf{\bar{O}}_{t-k-1}\}$. We explore three potential variants including \textit{recurrent}, \textit{rep-all}, and \textit{dense}, as shown in Fig. \ref{Fig.connection-form}

The \textit{recurrent} connection form utilizes information only from the last frame when inferring on current and previous frames, which can be formulated as:
\begin{equation}
    \mathbf{O}^{his}_{t-k} = \mathrm{Adaptor}(\mathbf{\bar{O}}_{t-k-1})
\end{equation}
where $\mathrm{Adaptor}$ is used to fit the history query into the current timestamp.

The \textit{rep-all} form instead leverages all available history information for the current frame and no history information for previous frames. The operation can be expressed as:
\begin{equation}
    \mathbf{O}^{his}_{t-k} = \left\{
\begin{array}{rcl}
        &\Phi,& k \ne 0 \\
        &\mathrm{Adaptor}(\{\mathbf{\bar{O}}_{t-N},...,\mathbf{\bar{O}}_{t-k-1}\}),&k = 0
\end{array} \right.
\end{equation}

Similar to \cite{densenet}, both current and previous frames use all available history information in the \textit{dense} connection form, which is expressed as:
\begin{equation}
    \mathbf{O}^{his}_{t-k} = \mathrm{Adaptor}(\{\mathbf{\bar{O}}_{t-N},...,\mathbf{\bar{O}}_{t-k-1}\})
\end{equation}

\begin{figure}[htbp]
\centering 
\includegraphics[width=0.4 \textwidth]{iccv2023Detection/fig/connection-form.pdf}
\caption{Three query connection forms. (a) Recurrent. (b) rep-all. (c) Dense. } 
\label{Fig.connection-form} 
\end{figure}

